Learning Wi-Fi Connection Loss Predictions for Seamless Vertical Handovers Using Multipath TCP

We present a novel data-driven approach to perform smooth Wi-Fi/cellular handovers on smartphones. Our approach relies on data provided by multiple smartphone sensors (e.g., Wi-Fi RSSI, acceleration, compass, step counter, air pressure) to predict Wi-Fi connection loss and uses Multipath TCP to dynamically switch between different connectivity modes. We train a random forest classifier and an artificial neural network on real-world sensor data collected by five smartphone users over a period of three months. The trained models are executed on smartphones to reliably predict Wi-Fi connection loss 15 seconds ahead of time, with a precision of up to 0.97 and a recall of up to 0.98. Furthermore, we present results for four DASH video streaming experiments that run on a Nexus 5 smartphone using available Wi-Fi/cellular networks. The neural network predictions for Wi-Fi connection loss are used to establish MPTCP subflows on the cellular link. The experiments show that our approach provides seamless wireless connectivity, improves quality of experience of DASH video streaming, and requires less cellular data compared to handover approaches without Wi-Fi connection loss predictions.

==> 4c_overhead.tex <==

\subsection{Overhead Analysis}

\begin{figure}[t]
    \centering
    \includegraphics[width=.95\columnwidth]{figures/energy}
    \caption{Power Consumption}
    \label{fig:energy_overhead}
\end{figure}

Executing a neural network on a mobile device introduces overhead in terms of CPU and memory usage, which is mainly reflected in power consumption.
To evaluate this overhead, power measurements were performed on a Nexus 5 smartphone.
To avoid interferences from the battery, we removed the battery from the device, soldered wires to the charge controller and put it back into the Nexus 5.
Then, we powered and measured the device using a Monsoon High Voltage Power Monitor\footnote{https://www.msoon.com/} with a sample rate of 5 kHz and a resolution of 286 $\mu$A.
The voltage was set to 4.2 V, which corresponds to about 92\% battery capacity.

Since the measured device was not mobile anymore due to the wired power setup, we performed a series of independent tests that are illustrated in Figure~\ref{fig:energy_overhead}.
First, we performed a baseline measurement using only Wi-Fi, where neither the on-device prediction nor the sensor logging was enabled (denoted as \emph{Wi-Fi}).
The second experiment additionally incorporated cellular connectivity (marked as \emph{MPTCP}).
During the last experiment, the Wi-Fi connection loss prediction (\emph{Seamless}) was measured.
In all tests, the video was streamed on the device as in all other tests (see Sec.~\ref{sec:eval2}.
Furthermore, the MPTCP kernel was used in all experiments.
The x-axis of Figure~\ref{fig:energy_overhead} shows the time in seconds and the y-axis denotes the consumed power in mW.
All tests were executed for 120 seconds, whereas in the prediction test the first 60 seconds were used for filling the observation window and the prediction started at $p_{start}$.

The average power consumption during the Wi-Fi tests is about 1856 mW with a standard deviation of 145 mW.
Enabling LTE on the device, the average power consumption increases by 18.9\% to about 2289 mW and a standard deviation of 143 mW.

The power consumption using our prediction approach depends on the current state.
During the first 60 seconds, LTE was enabled.
Here, the average consumption is about 2792 mW, which is about 22\% higher than during the MPTCP test.
Shortly after $p_{start}$, no Wi-Fi connection loss is predicted, thus the LTE is switched off, which causes the device to change routing tables, turn the LTE device off, and MPTCP has to reschedule its subflows.
Doing this increases the power consumption to an average of 2843 mW.
At $p_{tr.}$, the transition from MPTCP over Wi-Fi and LTE to Wi-Fi only has finished, so that the power usage decreases to about 2420 mW.
Compared to the consumption during the Wi-Fi tests, this is an overhead of 30.6\%.
Compared to the MPTCP test, the prediction introduces an overhead of 5.7\%.
In total, to retain the same high QoE, our approach introduces an overhead of 15.7\% on average (2649 mW, 300 mW standard deviation), including all three phases of the \textit{Seamless} tests.

Considering the 9660 mWh battery of the Nexus 5, the video could be streamed for about 4.22 hours continuously using MPTCP.
Incorporating our on-device prediction, the time decreases to 3.65 hours, which are about 34 minutes less watching time.
This is a reasonable overhead for executing a neural network in an Android app, and it can be further improved. For example,
Graubner et al. ~\cite{graubner2018multimodal} showed that certain computations can be performed in an energy-efficient manner by executing them on a mobile device's sensor hub or Wi-Fi chip.
%Since the main goal of this work is to increase the users' QoE in handover situations, an energy efficient implementation was out of scope for this work.
